A priori error estimates for finite element discretization of semilinear elliptic equations with non-Lipschitz nonlinearities

In this paper we develop numerical analysis for finite element discretization of semilinear elliptic equations with potentially non-Lipschitz nonlinearites. The nonlinearity is essecially assumed to be continuous and monotonically decreasing including the case of non-Lipschitz or even non-H\"older continuous nonlinearities. For a direct discretization (without any regularization) with linear finite elements we derive error estimates with respect to various norms and illustrate these results with a numerical example.

==> macros.tex <==
\newcommand{\N}{\varmathbb{N}}
\newcommand{\Z}{\varmathbb{Z}}
\newcommand{\Q}{\varmathbb{Q}}
\newcommand{\R}{\varmathbb{R}}
\newcommand{\C}{\varmathbb{C}}
\newcommand{\RR}{\mathcal R}
\newcommand{\B}{\mathcal B}
\newcommand{\NN}{{\mathcal N}}
\newcommand{\EE}{{\mathcal E}}
\renewcommand{\P}{{\mathcal P}}
\renewcommand{\L}{{\mathcal L}}
\newcommand{\OO}{{\mathcal O}}
\newcommand{\oo}{{\mathcal o}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normV}[1]{\norm{#1}_V}
\newcommand{\Mnorm}[1]{\Norm{#1}_{\M(\Omega)}}
\newcommand{\mnorm}[1]{\norm{#1}_{\M(\Omega)}}
\newcommand{\mnormc}[1]{\norm{#1}_{\M(\Omega_{\mathrm{c}})}}
\newcommand{\snorm}[1]{|#1|}
\newcommand{\ltwonorm}[1]{\norm{#1}_{L^2(\Omega)}}
\newcommand{\ltwonormdo}[1]{\norm{#1}_{L^2(\partial \Omega)}}
\newcommand{\ltwonormo}[1]{\norm{#1}_{L^2(\Omega_{\mathrm{o}})}}
\newcommand{\ltwonorms}[1]{\norm{#1}_{L^2(\omega)}}
\newcommand{\ltwonormh}[1]{\norm{#1}_{L^2(\Omega),h}}
\newcommand{\Ltwonorm}[1]{\Norm{#1}_{L^2(\Omega)}}
\newcommand{\Lpnorm}[1]{\Norm{#1}_{L^p(\Omega)}}
\newcommand{\honenorm}[1]{\norm{#1}_{H^1(\Omega)}}
\newcommand{\htwonorm}[1]{\norm{#1}_{H^2(\Omega)}}
\newcommand{\woneinfnorm}[1]{\norm{#1}_{W^{1,\infty}(\Omega)}}
\newcommand{\conegammanorm}[1]{\norm{#1}_{C^{1,\gamma}(\bar \Omega)}}
\newcommand{\lpnorm}[1]{\norm{#1}_{L^p(\Omega)}}
\newcommand{\lppnorm}[1]{\norm{#1}_{L^{p'}(\Omega)}}
\newcommand{\lonenorm}[1]{\norm{#1}_{L^1(\Omega)}}
\newcommand{\lonenormk}[1]{\norm{#1}_{L^1(K)}}
\newcommand{\lqnorm}[1]{\norm{#1}_{L^q(\Omega)}}
\newcommand{\ltwonormk}[1]{\norm{#1}_{L^2(K)}}
\newcommand{\lpnormk}[1]{\norm{#1}_{L^p(K)}}
\newcommand{\lqnormk}[1]{\norm{#1}_{L^q(K)}}
\newcommand{\ltwonorme}[1]{\norm{#1}_{L^2(E)}}
\newcommand{\linfnorm}[1]{\norm{#1}_{L^\infty(\Omega)}}
\newcommand{\linfnormdo}[1]{\norm{#1}_{L^\infty(\partial \Omega)}}
\newcommand{\linfnorms}[1]{\norm{#1}_{L^\infty(\omega)}}
\newcommand{\Linfnorm}[1]{\Norm{#1}_{L^\infty(\Omega)}}
\newcommand{\linfnormnull}[1]{\norm{#1}_{L^\infty(\Omega_0)}}
\newcommand{\linfnormk}[1]{\norm{#1}_{L^\infty(K)}}
\newcommand{\CC}{{\mathcal C}}
\newcommand{\into}{\int_\Omega}
\newcommand{\intdo}{\int_{\partial \Omega}}
\newcommand{\intk}{\int_K}
\newcommand{\intdk}{\int_{\partial K}}
\newcommand{\inte}{\int_E}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\sgn}{\operatorname{sgn}}
%\newcommand{\itemto}{\item[$\to$]}
%\newcommand{\itema}{\item[(a)]}
%\newcommand{\itemb}{\item[(b)]}
%\newcommand{\itemc}{\item[(c)]}
%\newcommand{\itemd}{\item[(d)]}
%\newcommand{\iteme}{\item[(e)]}
%\newcommand{\itemf}{\item[(f)]}
%\newcommand{\itemg}{\item[(g)]}
%\newcommand{\itemh}{\item[(h)]}
%\newcommand{\itemi}{\item[(i)]}
%\newcommand{\itemii}{\item[(ii)]}
%\newcommand{\itemiii}{\item[(iii)]}
%\newcommand{\itemiv}{\item[(iv)]}
%\newcommand{\itemdef}{\item[\textbf{Def.}]}
%\newcommand{\bi}{\begin{itemize}}
%\newcommand{\ei}{\end{itemize}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\nhalf}{\nicefrac{1}{2}}
\newcommand{\sumk}{\sum_{K\in \T_h}}
\newcommand{\sume}{\sum_{E\in \EE(\T_h)}}
\newcommand{\sumf}{\sum_{F\in {\mathcal F}(\T_h)}}
\newcommand{\sumek}{\sum_{E\in \EE(K)}}
\newcommand{\sumx}{\sum_{x\in \NN(\T_h)}}
\newcommand{\sumxk}{\sum_{x\in \NN(K)}}
\newcommand{\jump}{[n_E\cdot\nabla u_h]}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\arccot}{\operatorname{arccot}}
\newcommand{\Rang}{\operatorname{Rang}}
\newcommand{\Kern}{\operatorname{Kern}}
\newcommand{\Bild}{\operatorname{Bild}}
\newcommand{\Lin}{\operatorname{Lin}}
\newcommand{\sign}{\operatorname{sign}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\esssup}{\operatorname*{ess\,sup}}
\newcommand{\osc}{\operatorname{osc}}
\newcommand{\tnorm}[1]{|\mspace{-1.5mu}|\mspace{-1.5mu}|#1|\mspace{-1.5mu}|\mspace{-1.5mu}|}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\newcommand{\eps}{\varepsilon}

\newcommand{\Qad}{{Q_\mathrm{ad}}}
\newcommand{\Qadh}{{Q_{\mathrm{ad},h}}}
\newcommand{\Qadhc}{{Q^0_{\mathrm{ad},h}}}
\newcommand{\Qadhl}{{Q^1_{\mathrm{ad},h}}}
\newcommand{\Vad}{{V_\mathrm{ad}}}
\newcommand{\Vadh}{{V_{\mathrm{ad},h}}}
\newcommand{\oq}{\bar q}
\newcommand{\ou}{\bar u}
\newcommand{\oz}{\bar z}
\newcommand{\ox}{\bar x}
\newcommand{\omu}{\bar \mu}
\newcommand{\obeta}{\bar \beta}

\newcommand{\oqah}{\bar q_{\alpha,h}}
\newcommand{\ouah}{\bar u_{\alpha,h}}
\newcommand{\ozah}{\bar z_{\alpha,h}}


\newcommand{\dq}{\delta\mspace{-2mu}q}
\newcommand{\du}{\delta\mspace{-2mu}u}
\newcommand{\tdu}{\delta\mspace{-2mu}\tilde u}
\newcommand{\dz}{\delta\mspace{-2mu}z}

\newcommand{\dtu}{\delta\tau\mspace{-2mu}u}
\newcommand{\ddu}{\delta^2\mspace{-2mu}u}

\newcommand{\tq}{\tau\mspace{-2mu}q}
\newcommand{\tu}{\tau\mspace{-2mu}u}
\newcommand{\tz}{\tau\mspace{-2mu}z}

\newcommand{\M}{{\mathcal M}}

\newcommand{\lh}{\abs{\ln h}}
\newcommand{\Lap}{\upDelta}
\renewcommand{\phi}{\varphi}
\newcommand{\Om}{\Omega}
\newcommand{\Omc}{\Omega_{\mathrm{c}}}
\newcommand{\barOmc}{\bar\Omega_{\mathrm{c}}}
\newcommand{\Omo}{\Omega_{\mathrm{o}}}
\newcommand{\barOmo}{\bar\Omega_{\mathrm{o}}}

\newcommand{\rightharpoonupweak}{\mathrel{\ensurestackMath{\stackon[0.5pt]{\rightharpoonup}{\scriptstyle\ast}}}}
\newcommand{\weakto}{\rightharpoonup}
\newcommand{\hookrightarrowcompact}{\mathrel{\ensurestackMath{\stackon[0.5pt]{\hookrightarrow}{\scriptstyle c}}}}

\newcommand{\logLogSlopeTriangle}[6]
{
  % #1. Relative offset in x direction.
  % #2. Width in x direction, so xA-xB.
  % #3. Relative offset in y direction.
  % #4. Slope d(y)/d(log10(x)).
  % #5. Plot options.
  % #6. Text.

  \pgfplotsextra
  {
    \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
    \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
    \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
    \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

    \pgfmathsetmacro{\xArel}{#1}
    \pgfmathsetmacro{\yArel}{#3}
    \pgfmathsetmacro{\xBrel}{#1-#2}
    \pgfmathsetmacro{\yBrel}{\yArel}
    \pgfmathsetmacro{\xCrel}{\xArel}

    \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
    \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
    \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
    \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
    \pgfmathsetmacro{\yCrel}{(\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

    \coordinate (A) at (rel axis cs:\xArel,\yArel);
    \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
    \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

    \draw[#5]   (A)-- %node[pos=0.5,anchor=north] {1}
    (B)-- 
    (C)-- node[pos=0.5,anchor=west] {$#6$}
    cycle;
  }
}

\newcommand{\logLogSlopeTriangleInverse}[6]
{
  % #1. Relative offset in x direction.
  % #2. Width in x direction, so xA-xB.
  % #3. Relative offset in y direction.
  % #4. Slope d(y)/d(log10(x)).
  % #5. Plot options.
  % #6. Text.

  \pgfplotsextra
  {
    \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
    \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
    \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
    \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

    \pgfmathsetmacro{\xArel}{#1}
    \pgfmathsetmacro{\yArel}{#3}
    \pgfmathsetmacro{\xBrel}{#1-#2}
    \pgfmathsetmacro{\yBrel}{\yArel}
    \pgfmathsetmacro{\xCrel}{\xBrel}

    \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
    \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
    \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
    \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
    \pgfmathsetmacro{\yCrel}{2*\yArel-(\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

    \coordinate (A) at (rel axis cs:\xArel,\yArel);
    \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
    \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

    \draw[#5]   (A)-- %node[pos=0.5,anchor=north] {1}
    (B)-- node[pos=0.5,left,anchor=east] {$#6$}
    (C)-- 
    cycle;
  }
}

\newcommand{\itemEq}[1]{%
  \begingroup%
  \setlength{\abovedisplayskip}{2pt}%
  \setlength{\belowdisplayskip}{2pt}%
  \setlength{\abovedisplayshortskip}{2pt}%
  \setlength{\belowdisplayshortskip}{2pt}%
  \parbox[c]{\linewidth}{#1}%
\endgroup}


% Style to select only points from #1 to #2 (inclusive)
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}

